An Economic Model for Quantum Key-Recovery Attacks against Ideal Ciphers

It has been established that quantum algorithms can solve several key cryptographic problems more efficiently than classical computers. As progress continues in the field of quantum computing it is important to understand the risks they pose to deployed cryptographic systems. Here we focus on one of these risks - quantum key-recovery attacks against ideal ciphers. Specifically, we seek to model the risk posed by an economically motivated quantum attacker who will choose to run a quantum key-recovery attack against an ideal cipher if the cost to recover the secret key is less than the value of the information at the time when the key-recovery attack is complete. In our analysis we introduce the concept of a quantum cipher circuit year to measure the cost of a quantum attack. This concept can be used to model the inherent tradeoff between the total time to run a quantum key recovery attack and the total work required to run said attack. Our model incorporates the time value of the encrypted information to predict whether any time/work tradeoff results in a key-recovery attack with positive utility for the attacker. We make these predictions under various projections of advances in quantum computing. We use these predictions to make recommendations for the future use and deployment of symmetric key ciphers to secure information against these quantum key-recovery attacks. We argue that, even with optimistic predictions for advances in quantum computing, 128 bit keys (as used in common cipher implementations like AES-128) provide adequate security against quantum attacks in almost all use cases.

==> reverse.tex <==
%!TEX root=main.tex
Under the assumptions from our three worlds of quantum development we found that any quantum key recovery attack for a 128-bit key is not economically feasible. Here we seek to answer a related question: If we want an economically feasible attack, what kind of quantum computer would be required? We follow a similar strategy of proposing three attacks, but note that this analysis works for any relevant parameters. We begin here not by assuming any level of advancement in quantum computing but by assuming an attacked values some piece of information at a particular level. Here we select USD 100,000, 1,000,000, and 10,000,000 as the value of information. We also allow the attacker to select 1, 10, and 100 year attacks in the same manner as in Section \ref{sec:econ}.
When we set the cost and time limit for these attacks we arrive not at a single quantum computer that would suffice to run the attack but a family of quantum computers with varying speeds and costs. This fact arises from the theoretical ability to bring cost per cubit down if we allow for a computer to have a higher clock speed. So, when we set the total budget and time limit for an attack we arrive at some family of computers described in terms of the cost/speed tradeoffs. These tradeoffs are subject to the quadratic increase in cost seen when increasing the level of parallelism.
We denote a family of quantum computers $\mathcal{Q}_{b,T_y,n}$ based on a budget $b$, time limit in years $T_y$, and key length $n$. This describes the set of quantum computers capable of running a quantum key-recovery attack with the relevant restrictions. The family contains all quantum computers satisfying the property: $\mathcal{Q}_{b,T_y,n} = \left\{q : C_{CCY} \leq \frac{16b\left(\frac{\sigma}{d}\right)^2}{\pi^2 2^n T_y}\right\}$ where $d$ is the depth of the oracle circuit and $\sigma$ is the number of circuit layers that can be processed in the given time limit. 
We can now begin to look at some families of quantum computers based on some reasonable attack budgets. Consider an attack that is of vital importance - where an attacker is willing to spend USD 100 million on an attack on AES-128, and needs it within 100 years. A quantum computer capable of doing so is in $\mathcal{Q}_{1.0 \times 10^8,100,128}$, which contains all quantum computers such that $C_{CCY} \leq \frac{1.6 \times 10^9 \left(\frac{\sigma}{15040}\right)^2}{\pi^2 2^{128} 100} = 2.11 \times 10^{-41} \sigma^2$. Consider a case where we would like $C_{CCY} \leq USD 1000$. This would require the computer to run at a speed that computes $\sigma = 6.89 \times 10^{21}$ layers over 100 years, corresponding to a clock speed of $2.185 \times 10^{12}Hz$. This greatly exceeds even NIST's most optimistic predictions~\cite{nist_call_for_pqc}.  Any required parameters might be inserted here to see what would be required to make the existing parameters work - a plot of the family that can solve this problem is shown in Fig \ref{fig:speedcosttradeoff}. We note that no matter which parameters you pick for this attack you end up with a computer that is either impossibly fast or impossibly cheap, meaning that no quantum computer that can run an attack with this requested budget and time limit is feasible.

\begin{figure}
\begin{tikzpicture}
\usepgfplotslibrary{fillbetween}
\begin{loglogaxis}[
	xlabel=$\sigma (Hz)$,
	ylabel=$C_{CCY} (USD)$,	
	title=Speed vs QC CCY cost,
	enlarge x limits=false,
	axis on top,
]
\addplot[
	color = blue,
	domain=1e10:1e50,
	fill = blue!30!white
]{2.11e-41 * x^2} -- (rel axis cs:1,0) -- (rel axis cs:0,0);


\end{loglogaxis}
\end{tikzpicture}
\caption{Possible values of $C_{CCY}$ based on estimated QC speed ($b = 1.0 \times 10^8, T_y = 100, n=128$\label{fig:speedcosttradeoff}}
\end{figure}


%We begin by examining threshold attacks. As we %have noted in this model the optimal attack uses %the full time for the attack. 
%\begin{table} \centering
%\caption{QC Clock Speed Requirements (n = 128, %$T-y$ = 100 years) \label{tab:clockspeed}}
%\begin{tabular}{|l|c|}
%\hline
%Budget (USD) & $\mathcal{Q}_{b,T_y,n}$ \\ \hline
%1 million	&	$C_{CCY} \leq \frac{1.6 \times %10^6 \left(\frac{\sigma}{d}\right)^2}{\pi^2 2^n %T_y}\right\}$\\ \hline
%10 million & blah\\ \hline 
%100 million & blah\\ \hline
%\end{tabular}
%\end{table}
